High-harmonic spectroscopy of two-dimensional materials

Recent advancements in the generation of mid-infrared and terahertz laser pulses have enabled us to observe strong-field driven non-perturbative high-harmonic generation (HHG) from semiconductors, dielectrics, and semimetals. HHG has added another dimension to time-resolved ultrafast electron dynamics in materials with unprecedented temporal resolution. Present thesis discusses how HHG is an emerging method to probe static and dynamical properties in two-dimensional materials. In this thesis, two-dimensional materials with hexagonal symmetry are studied. We have demonstrated that the high-harmonic spectrum encodes the fingerprints of electronic band structure and interband coupling between different bands. Furthermore, by analysing gapped and gapless graphene, we show how electron dynamics in a semimetal and a semiconductor are different as the harmonic spectrum depends differently on the polarisation of the driving laser. To explore the role of defects in HHG, spin-polarised vacancy defects in hexagonal boron nitride are considered. It has been found that electron-electron interaction is crucial for electron dynamics in a defected solid. In all cases, we present how different symmetries of the lattice can be extracted from the harmonic spectrum. Finally, a light-driven method is proposed for observing valley-polarisation in pristine graphene, using a tailored laser pulse. Also, a recipe is discussed to write and read valley-selective electron excitations in materials with zero bandgap and zero Berry curvature.

==> HeadTail/certi.tex <==
\newpage
\thispagestyle{empty}
 \vspace*{2cm}
\begin{center}
\textbf{\Large\underline {Approval Sheet}}
\end{center}
\vspace{1cm}
This thesis entitled \textbf{High-harmonic Spectroscopy of Two-dimensional Materials} by \textbf{Mrudul M. S.} (Roll No. 164120007) is approved for the degree of Doctor of Philosophy in Physics.

\begin{flushright}
\textbf{Examiners}\\
\-------------------------\\
\-------------------------\\
\-------------------------\\



\textbf{Supervisor}\\
Dr. Gopal Dixit

\textbf{Chairman}\\
\-------------------------\\


\end{flushright}

\begin{flushleft}
Date :\\
Place :
\end{flushleft}


